Future-Conditioned Recommendations with Multi-Objective Controllable Decision Transformer

Securing long-term success is the ultimate aim of recommender systems, demanding strategies capable of foreseeing and shaping the impact of decisions on future user satisfaction. Current recommendation strategies grapple with two significant hurdles. Firstly, the future impacts of recommendation decisions remain obscured, rendering it impractical to evaluate them through direct optimization of immediate metrics. Secondly, conflicts often emerge between multiple objectives, like enhancing accuracy versus exploring diverse recommendations. Existing strategies, trapped in a "training, evaluation, and retraining" loop, grow more labor-intensive as objectives evolve. To address these challenges, we introduce a future-conditioned strategy for multi-objective controllable recommendations, allowing for the direct specification of future objectives and empowering the model to generate item sequences that align with these goals autoregressively. We present the Multi-Objective Controllable Decision Transformer (MocDT), an offline Reinforcement Learning (RL) model capable of autonomously learning the mapping from multiple objectives to item sequences, leveraging extensive offline data. Consequently, it can produce recommendations tailored to any specified objectives during the inference stage. Our empirical findings emphasize the controllable recommendation strategy's ability to produce item sequences according to different objectives while maintaining performance that is competitive with current recommendation strategies across various objectives.

==> sections/author.tex <==

\author{Chongming Gao}
\email{chongming.gao@gmail.com}
\orcid{0000-0002-5187-9196}
\affiliation{%
  \institution{University of Science and Technology of China}
%   \streetaddress{P.O. Box 1212}
  \city{Hefei}
  \state{Anhui}
  \country{China}
%   \postcode{43017-6221}
}


\author{Kexin Huang}
\email{huangkx@mail.ustc.edu.cn}
\orcid{0009-0001-4868-0952}
\affiliation{%
  \institution{University of Science and Technology of China}
%   \streetaddress{P.O. Box 1212}
  \city{Hefei}
  \state{Anhui}
  \country{China}
%   \postcode{43017-6221}
}


\author{Zian Fei}
\email{feiziang@mail.ustc.edu.cn}
% \orcid{0000-0002-7849-208X}
\affiliation{%
  \institution{University of Science and Technology of China}
  \city{Hefei}
  \state{Anhui}
  \country{China}
}


\author{Jiaju Chen}
\email{cjj01@mail.ustc.edu.cn}
% \orcid{0000-0001-5667-5347}
\affiliation{%
  \institution{University of Science and Technology of China}
  \city{Hefei}
  \state{Anhui}
  \country{China}
}


\author{Jiawei Chen}
\email{sleepyhunt@zju.edu.cn}
\orcid{0000-0002-4752-2629}
\affiliation{%
  \institution{Zhejiang University}
%   \streetaddress{P.O. Box 1212}
  \city{Hangzhou}
  \state{Zhejiang}
  \country{China}
%   \postcode{43017-6221}
}


% \author{Peng Jiang}
% \email{jiangpeng@kuaishou.com}
% \orcid{0000-0002-9266-0780}
% \affiliation{%
%   \institution{Kuaishou Technology Co., Ltd.}
%   \country{}
% }

% \author{Shiqi Wang}
% \email{shiqi@cqu.edu.cn}
% \orcid{0000-0002-5369-884X}
% \affiliation{%
%   \institution{Chongqing University}
%   \city{Chongqing}
%   \country{China}
% }

% \author{Zhong Zhang}
% \email{zhongzhang@std.uestc.edu.cn}
% \orcid{0000-0003-1349-9755}
% \affiliation{%
%   \institution{University of Electronic Science and Technology of China}
%   \country{}
% }


% \author{Xiangnan He}
% \authornotemark[1]
% \email{xiangnanhe@gmail.com}
% \orcid{0000-0001-8472-7992}
% \affiliation{%
%   \institution{University of Science and Technology of China}
%   \country{}
% }

\renewcommand{\shortauthors}{Chongming Gao et al.}

% \renewcommand{\shortauthors}{Gao et al.}

==> sections/definition.tex <==
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    Bib\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{XXXXXXX.XXXXXXX}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[Conference acronym 'XX]{Make sure to enter the correct
  conference title from your rights confirmation emai}{June 03--05,
  2018}{Woodstock, NY}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}



\usepackage{booktabs}
\usepackage{multirow}
\usepackage{url}
\usepackage{enumitem}   
\usepackage{float} % For figure floating in appendix
\usepackage{colortbl} % 引入colortbl包
\definecolor{mygray}{rgb}{0.9, 0.9, 0.9}




\definecolor{myred}{rgb}{0.68627451, 0.14117647, 0.09803922}

% Added automatically
% \newcommand{\myeq}[1]{\hyperref[eq:#1]{Equation~(\ref*{eq:#1})}}
\newcommand{\myeq}[1]{\hyperref[eq:#1]{Eq.~(\ref*{eq:#1})}}
\newcommand{\mysec}[1]{\hyperref[sec:#1]{Section~\ref*{sec:#1}}}
\newcommand{\mytable}[1]{\hyperref[tab:#1]{Table~\ref*{tab:#1}}}
\newcommand{\myfig}[1]{\hyperref[fig:#1]{Fig.~\ref*{fig:#1}}}
\newcommand{\myappendix}[1]{\hyperref[appendix:#1]{Appendix~\ref*{appendix:#1}}}
% \newcommand{\myappendix}[1]{\hyperref[appendix:#1]{Appendix}}
\newcommand{\myalg}[1]{\hyperref[alg:#1]{Algorithm~\ref*{alg:#1}}}
\newcommand{\myhyp}[1]{\hyperref[hyp:#1]{\textsc{Hypothesis}~\ref*{hyp:#1}}}


\newcommand{\mytheorem}[1]{\hyperref[theorem:#1]{Theorem~\ref*{theorem:#1}}}
\newcommand{\mylemma}[1]{\hyperref[lemma:#1]{Lemma~\ref*{lemma:#1}}}
%



==> sections/meta.tex <==
% \copyrightyear{2022}
% \acmYear{2022}
% \setcopyright{acmcopyright}
% \acmConference[SIGIR '23] {Proceedings of the 46th International ACM SIGIR Conference on Research and Development in Information Retrieval}{July 23--27, 2023}{Taipei.}
% \acmBooktitle{Proceedings of the 46th International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR '23), July 23--27, 2023, Taipei.}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-9236-5/22/10}
% \acmDOI{10.1145/3511808.3557624}

% % SIGIR 23
% \copyrightyear{2023} 
% \acmYear{2023} 
% \setcopyright{acmlicensed}\acmConference[SIGIR '23]{Proceedings of the 46th
% International ACM SIGIR Conference on Research and Development in
% Information Retrieval}{July 23--27, 2023}{Taipei, Taiwan}
% \acmBooktitle{Proceedings of the 46th International ACM SIGIR Conference on
% Research and Development in Information Retrieval (SIGIR '23), July 23--27,
% 2023, Taipei, Taiwan}
% \acmPrice{15.00}
% \acmDOI{10.1145/3539618.3591636}
% \acmISBN{978-1-4503-9408-6/23/07}




\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10003317.10003347.10003350</concept_id>
<concept_desc>Information systems~Recommender systems</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}
\ccsdesc[500]{Information systems~Recommender systems}


% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>00000000.0000000.0000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Do, Not, Us, This, Code, Put, the, Correct, Terms, for,
  Your, Paper}

% %% A "teaser" image appears between the author and affiliation
% %% information and the body of the document, and typically spans the
% %% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

